Nonstationary, Nonparametric, Nonseparable Bayesian Spatio-Temporal Modeling Using Kernel Convolution of Order Based Dependent Dirichlet Process

In this article, using kernel convolution of order based dependent Dirichlet process (Griffin and Steel (2006)) we construct a nonstationary, nonseparable, nonparametric space-time process, which, as we show, satisfies desirable properties, and includes the stationary, separable, parametric processes as special cases. We also investigate the smoothness properties of our proposed model. Since our model entails an infinite random series, for Bayesian model fitting purpose we must either truncate the series or more appropriately consider a random number of summands, which renders the model dimension a random variable. We attack the variable dimensionality problem using Transdimensional Transformation based Markov Chain Monte Carlo introduced by Das and Bhattacharya (2019b), which can update all the variables and also change dimensions in a single block using essentially a single random variable drawn from some arbitrary density defined on a relevant support. For the sake of completeness we also address the problem of truncating the infinite series by providing a uniform bound on the error incurred by truncating the infinite series. We illustrate the effectiveness of our model and methodologies on a simulated data set and demonstrate that our approach significantly outperforms that of Fuentes and Reich (2013) which is based on principles somewhat similar to ours. We also fit two real, spatial and spatio-temporal datasets with our approach and obtain quite encouraging results in both the cases.

==> figures.tex <==

\begin{figure}[htb]
%\begin{center}
\centering
\includegraphics[height=1.5in,width=2.1in]{plots_final_time/y_1_time.pdf}
\includegraphics[height=1.5in,width=2.1in]{plots_final_time/y_12_time.pdf}
\includegraphics[height=1.5in,width=2.1in]{plots_final_time/y_50_time.pdf}
\includegraphics[height=1.5in,width=2.1in]{plots_final_time/y_53_time.pdf}
\includegraphics[height=1.5in,width=2.1in]{plots_final_time/y_67_time.pdf}
\includegraphics[height=1.5in,width=2.1in]{plots_final_time/y_95_time.pdf}
\caption{Simulation study: Posterior predictive densities of $Y(\bs,t)$ for 6 different location-time pairs 
-- the corresponding true values
are denoted by the vertical line.}
\label{fig:posterior_predictive2}
%\end{center}
\end{figure}


\begin{figure}[htb]
%\begin{center}
\centering
\includegraphics[height=1.5in,width=2.1in]{correlation_plots/correlation_1_2-crop.pdf}
\includegraphics[height=1.5in,width=2.1in]{correlation_plots/correlation_1_7-crop.pdf}
\includegraphics[height=1.5in,width=2.1in]{correlation_plots/correlation_1_95-crop.pdf}
\\[5mm]
\includegraphics[height=1.5in,width=2.1in]{correlation_plots/correlation_5_9-crop.pdf}
\includegraphics[height=1.5in,width=2.1in]{correlation_plots/correlation_5_12-crop.pdf}
\includegraphics[height=1.5in,width=2.1in]{correlation_plots/correlation_5_91-crop.pdf}
\\[5mm]
\includegraphics[height=1.5in,width=2.1in]{correlation_plots/correlation_21_23-crop.pdf}
\includegraphics[height=1.5in,width=2.1in]{correlation_plots/correlation_21_55-crop.pdf}
\includegraphics[height=1.5in,width=2.1in]{correlation_plots/correlation_21_92-crop.pdf}
\\[5mm]
\includegraphics[height=1.5in,width=2.1in]{correlation_plots/correlation_60_10-crop.pdf}
\includegraphics[height=1.5in,width=2.1in]{correlation_plots/correlation_60_69-crop.pdf}
\includegraphics[height=1.5in,width=2.1in]{correlation_plots/correlation_60_95-crop.pdf}
\caption{Simulation study: Posterior densities of correlations for 12 different pairs of locations; the vertical lines 
indicate the true correlations.}
\label{fig:correlation}
%\end{center}
\end{figure}


\begin{figure}[htb]
%\begin{center}
\centering
\includegraphics[height=3in,width=4in]{plots_final_real/surface_real_data-crop}
\\[2cm]
\includegraphics[height=3in,width=4in]{plots_final_real/surface_real_median-crop}
\caption{Real data analysis: The top panel shows the surface plot of ozone concentrations (middle), the lower and the upper
95\% credible intervals associated with the leave-one-out posterior predictive densities, denoted
by the lower and the upper surfaces, respectively. The bottom panel shows the surface
plot of the posterior medians (middle) along with the lower and the upper 95\% credible intervals
associated with the leave-one-out posterior predictive densities (lower and the upper surfaces, respectively).
The observed data points are indicated by `*'.}
\label{fig:real_surface_plots}
%\end{center}
\end{figure}


%\newpage
%\begin{figure}[htb]
%%\begin{center}
%\centering
%\includegraphics[height=1.5in,width=2.1in]{plots_final_real/real_location1.pdf}
%\includegraphics[height=1.5in,width=2.1in]{plots_final_real/real_location39.pdf}
%\includegraphics[height=1.5in,width=2.1in]{plots_final_real/real_location50.pdf}
%\caption{Posterior Predictive Densities of Ozone Concentration at 3 different locations}
%\label{Fig2:Posterior Predictive at locations 1,39,50}
%%\end{center}
%\end{figure}
%
\begin{figure}[htb]
 \centering
\includegraphics[height=3in,width=6in]{plots_final_real/real_quantile.pdf}
\caption{Real data analysis: Posterior predictive distributions summarized by the median (middle line) and the $95\%$ credible intervals 
as a function of $\bs$. 
The observed data points are denoted by `*'.  }
\label{fig:median}
%\end{center}
\end{figure}


\begin{figure}[htb]
%\begin{center}
\centering
\includegraphics[height=1.5in,width=2.1in]{correlation_plots_real/correlation_1_5_real-crop.pdf}
\includegraphics[height=1.5in,width=2.1in]{correlation_plots_real/correlation_4_21_real-crop.pdf}
\includegraphics[height=1.5in,width=2.1in]{correlation_plots_real/correlation_4_75_real-crop.pdf}
\\[5mm]
\includegraphics[height=1.5in,width=2.1in]{correlation_plots_real/correlation_25_55_real-crop.pdf}
\includegraphics[height=1.5in,width=2.1in]{correlation_plots_real/correlation_35_45_real-crop.pdf}
\includegraphics[height=1.5in,width=2.1in]{correlation_plots_real/correlation_55_67_real-crop.pdf}
\caption{Real data analysis: Posterior densities of correlations for 6 different pairs of locations.}
\label{fig:correlation_real}
%\end{center}
\end{figure}


